Impact of classification difficulty on the weight matrices spectra in Deep Learning and application to early-stopping

Much research effort has been devoted to explaining the success of deep learning. Random Matrix Theory (RMT) provides an emerging way to this end: spectral analysis of large random matrices involved in a trained deep neural network (DNN) such as weight matrices or Hessian matrices with respect to the stochastic gradient descent algorithm. To have more comprehensive understanding of weight matrices spectra, we conduct extensive experiments on weight matrices in different modules, e.g., layers, networks and data sets. Following the previous work of \cite{martin2018implicit}, we classify the spectra in the terminal stage into three main types: Light Tail (LT), Bulk Transition period (BT) and Heavy Tail(HT). These different types, especially HT, implicitly indicate some regularization in the DNNs. A main contribution from the paper is that we identify the difficulty of the classification problem as a driving factor for the appearance of heavy tail in weight matrices spectra. Higher the classification difficulty, higher the chance for HT to appear. Moreover, the classification difficulty can be affected by the signal-to-noise ratio of the dataset, or by the complexity of the classification problem (complex features, large number of classes) as well. Leveraging on this finding, we further propose a spectral criterion to detect the appearance of heavy tails and use it to early stop the training process without testing data. Such early stopped DNNs have the merit of avoiding overfitting and unnecessary extra training while preserving a much comparable generalization ability. These findings from the paper are validated in several NNs, using Gaussian synthetic data and real data sets (MNIST and CIFAR10).

==> C06table.tex <==
\newgeometry{top=1.5cm}


\section{spectral criterion with 0.6}\label{sec: specrit}
\vspace{-3pt}
\begin{table}[htbp]
\centering
\caption{~~ Early stopping results in numeric experiments with $C=0.6$: stopping epochs selected by spectral criterion in different layers' weight matrices and their testing accuracy (Test Acc). The symbol ”-” means no early stopping epoch is found by the spectral criterion.\label{tbl:earlystoppingsimu1}}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination NN1+$\calD_1$}\\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Typical\\ TP\end{tabular}} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}          & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                                                                      & epoch(FC2)  & Test Acc & epoch(FC3)  & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
0.15                                                                  & 8           & 24.58\%  & 16          & 20.44\%  & HT        & HT       & 20.17\%       \\ \hline
0.2                                                                   & 8           & 31.50\%  & 16          & 25.83\%  & HT        & HT       & 27.03\%       \\ \hline
0.3                                                                   & 8           & 49.09\%  & 12          & 45.48\%  & HT        & HT       & 44.80\%       \\ \hline
0.6                                                                   & 9           & 87.96\%  & \multicolumn{2}{c|}{-} & BT       & BT      & 88.30\%       \\ \hline
0.9                                                                   & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & LT       & 99.13\%       \\ \hline
\end{tabular}
\vskip 2mm


\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination NN1+$\calD_2$}\\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Typical\\ TP\end{tabular}} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}  & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                                                                      & epoch(FC2)  & Test Acc  & epoch(FC3)  & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
0.24                                                                  & 9           & 14.69\%   & \multicolumn{2}{c|}{-} & HT        & HT       & 13.08\%       \\ \hline
1.2                                                                   & 8           & 39.31\%   & 16          & 32.11\%  & HT        & HT       & 32.98\%       \\ \hline
2.4                                                                   & 8           & 76.75\%   & 20          & 74.29\%  & HT        & HT       & 75.92\%       \\ \hline
3.2                                                                   & 10          & 91.94\%   & \multicolumn{2}{c|}{-} & HT        & LT      & 92.64\%       \\ \hline
4.8                                                                   & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & LT        & LT       & 99.73\%       \\ \hline
\end{tabular}

\vskip 2mm

\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination NN2+$\calD_1$}\\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Typical\\ TP\end{tabular}} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}  & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                                                                      & epoch(FC1)  & Test Acc  & epoch(FC2)  & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
0.02                                                                  & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & HT        & BT      & 16.02\%       \\ \hline
0.04                                                                  & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & HT        & BT      & 25.38\%       \\ \hline
0.07                                                                  & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & HT        & BT      & 50.12\%       \\ \hline
0.13                                                                  & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & BT       & LT       & 87.50\%       \\ \hline
0.2                                                                   & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & LT        & LT       & 99.14\%       \\ \hline
\end{tabular}
\vskip 2mm


\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination NN2+$\calD_2$}\\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Typical\\ TP\end{tabular}} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}  & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                                                                      & epoch(FC1)  & Test Acc  & epoch(FC2)  & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
0.24                                                                  & 12          & 13.48\%   & 7           & 13.19\%  & HT        & HT       & 13.44\%       \\ \hline
1.2                                                                   & 24          & 35.80\%   & 5           & 34.63\%  & HT        & HT       & 36.31\%       \\ \hline
2.4                                                                   & 6           & 73.80\%   & 36          & 74.86\%  & BT       & BT      & 75.12\%       \\ \hline
3.2                                                                   & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & LT        & LT       & 91.20\%       \\ \hline
4.8                                                                   & \multicolumn{2}{c|}{-}  & \multicolumn{2}{c|}{-} & LT        & LT       & 99.59\%         \\ \hline
\end{tabular}
\end{table}


















\vspace{-30pt}
\begin{table}[htbp]
\centering
\caption{~~  Early stopping results in real data experiments with $C=0.6$.\label{tbl:earlystopingreal1}}
\setlength{\textwidth}{1.5mm}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination LeNet+MNIST}\\
\hline
\multirow{2}{*}{batchsize} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}                 & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                           & epoch(FC1)  & Test Acc & epoch(FC2)  & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
16                         & \multicolumn{2}{c|}{-} & 32          & 99.19\%  & LT        & BT      & 99.17\%       \\ \hline
32                         & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & BT      & 99.17\%       \\ \hline
64                         & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & BT      & 98.98\%       \\ \hline
128                        & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & BT       & 99.03\%       \\ \hline
256                        & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & LT       & 98.96\%       \\ \hline
\end{tabular}}
\vskip 2mm
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination LeNet+CIFAR10}\\
\hline
\multirow{2}{*}{batchsize} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}              & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                           & epoch(FC1)  & Test Acc & epoch(FC2) & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
16                         & 28          & 61.66\%  & 8          & 61.62\%  & BT       & HT       & 64.99\%       \\ \hline
32                         & \multicolumn{2}{c|}{-} & 20         & 61.06\%  & BT        & HT       & 64.57\%       \\ \hline
64                         & \multicolumn{2}{c|}{-} & 32         & 60.27\%  & LT        & BT       & 62.49\%       \\ \hline
128                        & \multicolumn{2}{c|}{-} & 60         & 61.38\%  & LT        & BT       & 61.83\%       \\ \hline
256                        & \multicolumn{2}{c|}{-} & 92         & 58.33\%  & LT        & BT       & 60.49\%       \\ \hline
\end{tabular}

\vskip 2mm
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination MiniAlexNet+MNIST}\\
\hline
\multirow{2}{*}{batchsize} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}                 & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                           & epoch(FC1)  & Test Acc & epoch(FC2)  & Test Acc & FC1       & FC2      & Test Acc      \\ \hline
16                         & 5           & 98.64\%  & \multicolumn{2}{c|}{-} & BT       & LT       & 99.49\%       \\ \hline
32                         & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & BT        & LT       & 99.41\%       \\ \hline
64                         & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & LT       & 99.42\%       \\ \hline
128                        & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & LT       & 99.39\%       \\ \hline
256                        & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & LT        & LT       & 99.31\%       \\ \hline
\end{tabular}


\vskip 2mm
\setlength{\textwidth}{1.5mm}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{The combination MiniAlexNet+CIFAR10}\\
\hline
\multirow{2}{*}{batchsize} & \multicolumn{4}{c|}{spectral criterion $C=0.6$}              & \multicolumn{3}{c|}{Final Epoch 248} \\ \cline{2-8} 
                           & epoch(FC1) & Test Acc & epoch(FC2)  & Test Acc & FC1     & FC2     & Test Acc         \\ \hline
16                         & 4          & 71.01\%  & 36(RC)      & 55.6\%   & HT      & RC      & 10\%(explode)    \\ \hline
32                         & 4          & 72.17\%  & 196(RC)     & 62.84\%  & HT      & RC      & 10\%(explode)    \\ \hline
64                         & 6          & 73.03\%  & \multicolumn{2}{c|}{-} & BT      & BT      & 77.94\%          \\ \hline
128                        & 12         & 74.31\%  & \multicolumn{2}{c|}{-} & BT      & LT      & 77.43\%          \\ \hline
256                        & 28         & 75.87\%  & \multicolumn{2}{c|}{-} & BT     & LT      & 75.93\%          \\ \hline
\end{tabular}}
\end{table}






% \begin{table}[htbp]
% \centering

% \caption{~~Experiments on LeNet+MNIST: The whole training alarm never appears during training procedure except batchsize 16 in FC2, "-" means $\hs_n$ never touches the alarm line.}
% \label{LeMNIST06}
% \end{table}



% \begin{table}[htbp]
% \centering

% \caption{~~Experiments on MiniAlexNet+MNIST: The whole training alarm never appears during training procedure except batchsize 16 in FC1, "-" means $\hs_n$ never touches the alarm line.}
% \label{AlexMNIST06}
% \end{table}



% \begin{table}[htbp]
% \centering

% \caption{~~Experiments on LeNet+CIFAR10: Training alarm appears during training procedure especially in FC2, and testing accuracy at stopping epoch is close to the final testing accuracy. "-" means $\hs_n$ never touches the alarm line.}
% \label{LeCIFAR06}
% \end{table}



% \begin{table}[htbp]
% \centering

% \caption{~~Experiments on MiniAlexNet+CIFAR10: Training alarm appears during training procedure especially in FC1, and testing accuracy at stopping epoch is close to the final testing accuracy except batchsize 16 and 32. Testing accuracy equals to 10\% means that the training has been exploded. "-" means $\hs_n$ never touches the alarm line.}
% \label{AlexCIFAR06}
% \end{table}




==> algorithm.tex <==
\section{Algorithm} \label{sec:algo}
\begin{algorithm}
\caption{Auto Detection of spikes}\label{Detectspikes}
\begin{algorithmic}
\Require Eigenvalues $\{\lambda_i\}_{i=1}^N$, $\alpha\gets7$.
\State Sort $\lambda_i$ with descending order, $\lambda_i>\lambda_{i+1}$
\For{$i=1$; $i<N$; $i++$}
\State $\beta_i\gets \lambda_i-\lambda_{i+1}$
\EndFor

\State $\beta=\sum_{i=1}^{N-1}\beta_i/(N-1)$
\State $r\gets$ $\alpha\cdot\beta$

\For{$i=1$; $i<N/2$; $i++$}
\If{$\beta_i>r$}
\State HS $\gets i$
\EndIf
\EndFor

\For{$i=N-1$; $i>N/2$; $i--$}
\If{$\beta_i>r$}
\State TS $\gets N-i$
\EndIf
\EndFor
\State \Return HS,TS
\end{algorithmic}
\end{algorithm}

The Algorithm \ref{Detectspikes} gives us an automatic method of detecting spikes, without the spike eigenvalues, we could achieve the deviation measurement between ESDs in weight matrices and standard MP Law by Algorithm 2.

\begin{algorithm}
\caption{Get deviation measurement $\hs_n$}\label{DetectSn}
\begin{algorithmic}
\Require Eigenvalues $\{\lambda_i\}_{i=1}^N$, $\alpha\gets7$.
\State Sort $\lambda_i$ with descending order, $\lambda_i>\lambda_{i+1}$
\State HS,TS $\gets$ Algorithm \ref{Detectspikes}($\{\lambda_i\}_{i=1}^N$, $\alpha$)
\State $n\gets N-$HS$-$TS


\For{$i=1$; $i\leq n$; $i++$}
\State $\gamma_i\gets \lambda_{i+\text{HS}}$            \Comment Get eigenvalues lying in the bulk
\EndFor

\State $M\gets2\lfloor n^{\frac13}\rfloor$   \Comment The number of Bins
\State $H\gets \lfloor n/M\rfloor$
\State $f(x)\gets \frac{2\sqrt{(\gamma_1-x)(x-\gamma_n)}}{\pi(\sqrt{\gamma_1}-\sqrt{\gamma_n})^2x}$
\State $\hs_n=0$
\For{$i=1$; $i<M$; $i++$}
\State $a,b\gets (i-1)H+1,iH+1$
\State $L\gets(b-a)/n/(\gamma_a-\gamma_b)$
\State $s\gets\int_{\gamma_b}^{\gamma_a}|f(x)-L|dx$
\State $\hs_n\gets\hs_n+s$
\EndFor
\State $a,b\gets (M-1)H+1,n$
\State $L\gets(b-a)/n/(\gamma_a-\gamma_b)$
\State $s\gets\int_{\gamma_b}^{\gamma_a}|f(x)-L|dx$
\State $\hs_n\gets\hs_n+s$

\State \Return $\hs_n$
\end{algorithmic}
\end{algorithm}



==> batchtable.tex <==
\pagestyle{empty}
\begin{table}[htbp]
\centering
\caption{~~NN1+$\calD_1$: The results in different batch sizes. RC means Rank Collapse. }
\label{tb:batchNN1D1}
\begin{tabular}{|c|c|c|c|}
\hline
Batch Size           & Layer                & Transition Period & TP Range+ESD Type                                                                                                            \\ \hline
\multirow{9}{*}{256} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.16{]}: HT(0,0)\\ {[}0.17,0.22{]}: HT(0,8)\end{tabular}                                  \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.23,0.55{]}: HT(0,7)$\to$MPB(0,7)                                                                                        \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.56,2{]}: LT(1,7)                                                                                                        \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & -                                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.01,0.4{]}: MPB(1,7)                                                                                                     \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.41,1.01{]}: LT(1,7)\\ {[}1.02,1.95{]}: LT(0,8)\\ {[}2{]}: LT(0,7)\end{tabular}               \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.01,2{]}: LT(0,7) (RC$\to$MP)                                                                                            \\ \hline
\multirow{9}{*}{64}  & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.19{]}: HT(0,1)\\ {[}0.2,0.25{]}: HT(7,1)\\ {[}0.26,0.36{]}: HT(0,8)\end{tabular}        \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.37-0.72{]}: HT(1,7)$\to$MPB(1,7)                                                                                        \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.73,1.09{]}: LT(1,7)\\ {[}1.1,1.9{]}: LT(0,8)\\ {[}1.95,2{]}: LT(0,7)\end{tabular}            \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & {[}0.01,0.32{]}: HT(0,8)                                                                                                     \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.32,0.62{]}: HT(1,7)$\to$MPB(1,7)                                                                                        \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.63,1.15{]}: LT(1,7)\\ {[}1.16,1.95{]}: LT(0,8)\\ {[}2{]}: LT(0,7)\end{tabular}               \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.01,2{]}: LT(0,7) (RC$\to$MP)                                                                                            \\ \hline
\multirow{9}{*}{32}  & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.17{]}: HT(0,1)\\ {[}0.18,0.46{]}: HT(7,1)\\ {[}0.47,0.55{]}: HT(0,8)\end{tabular}       \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.56,0.8{]}: HT(1,7)$\to$MPB(0,7)                                                                                         \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.81,0.84{]}: LT(0,7)\\ {[}0.85,1.08{]}: LT(1,7)\\ {[}1.09,2{]}: LT(0,8)\end{tabular}          \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.44{]}: RC\\ {[}0.45,0.52{]}: HT(7,1)\\ {[}0.53,0.59{]}: HT(0,8)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.6,0.72{]}: HT(1,7)$\to$MPB(0,7)                                                                                         \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.73,0.78{]}: LT(0,7)\\ {[}0.79,1.12{]}: LT(1,7)\\ {[}1.13,2{]}: LT(0,8)\end{tabular}          \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.01,0.45{]}: HT(0,7)$\to$MPB(0,7) (RC)                                                                                   \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.46,2{]}: LT(0,7) (RC$\to$MP)                                                                                            \\ \hline
\end{tabular}

\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}




\begin{table}[htbp]
\centering
\caption{~~NN2+$\calD_2$: The results in different batch sizes.}
\label{tb:batchNN2D2}
\begin{tabular}{|c|c|c|c|}
\hline
Batch Size           & Layer                & Transition Period & TP Range+ESD Type                                                                           \\ \hline
\multirow{6}{*}{256} & \multirow{3}{*}{FC1} & Heavy Tail        & -                                                                                           \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                           \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,1.2{]}: LT(0,0)\\ {[}1.28,4.8{]}: LT(0,7)\end{tabular}   \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                           \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                           \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,4.64{]}: LT(1,7)\\ {[}4.72,4.8{]}: LT(0,8)\end{tabular}  \\ \hline
\multirow{6}{*}{64}  & \multirow{3}{*}{FC1} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,0.96{]}: HT(0,0)\\ {[}1.04,1.12{]}: HT(0,8)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}1.2,2.72{]}: HT(1,7)$\to$MPB(1,7)                                                        \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}2.8,3.04{]}: LT(1,7)\\ {[}3.12,4.8{]}: LT(0,7)\end{tabular}  \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                           \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,2.4{]}: MPB(1,7)                                                                  \\ \cline{3-4} 
                     &                      & Light Tail        & {[}2.48,4.8{]}: LT(1,7)$\to$LT(0,8)                                                      \\ \hline
\multirow{6}{*}{32}  & \multirow{3}{*}{FC1} & Heavy Tail        & {[}0.08,0.8{]}: HT(0,0)                                                                     \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.88,3.6{]}: HT(0,7)$\to$MPB(0,7)                                                        \\ \cline{3-4} 
                     &                      & Light Tail        & {[}3.68,4.8{]}: LT(0,7)                                                                     \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                           \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,3.28{]}: RC$\to$MPB(0,7)                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & {[}3.36,4.8{]}: LT(1,7)                                                                     \\ \hline
\end{tabular}

\end{table}
% \pagestyle{plain}

==> preliminaries.tex <==
\section{Preliminaries on RMT}\label{sec: RMT}
\pagestyle{plain}
In this section, we review the results we use from RMT. RMT provides us lots of analysis results for both square or rectangular large matrices.  The well-known results in RMT: Marchenko-Pauster (MP) Law which shows eigenvalues' distribution of rectangular matrices, and Tracy-Widom Law which describes how the max eigenvalue distributed. When analyze DNNs weight matrices, MP Law, which is applicable to rectangular matrices, will give guidance on the analysis in spectrum of DNNs weight matrices.

% \subsection{Gaussian model}
% Gaussian model is one of the most representative statistic models. In the multi-classification task, it is also the most common model we assume to take theoretical consideration. In Gaussian model, we assume the sample data $x_{i,k}=\mu_k+\varepsilon_{i,k}\in \bbR^p$, $\varepsilon_{i,k}\stackrel{iid}{\sim} \calN(0,I_p)$. Here, $p$ is the dimension of input data, $k\in\{1,...,K\}$ implies the true class which input data belongs, $i\in\{1,...,n_k\}$, $n_k$ is the number of sample data in class $k$, $\mu_k\in\bbR^p$ is the population mean vector of class $k$. We define $\mu_G=\ave\limits_{k}\mu_k$ and its second moment matrices, the total covariance matrix 
% $$
% \Sigma_T\Def\ave\limits_{i,k}(h_{i,k}-\mu_G)(h_{i,k}-\mu_G)^T,
% $$
% the between class covariance matrix
% $$
% \Sigma_B\Def\ave\limits_{k}(\mu_{k}-\mu_G)(\mu_k-\mu_G)^T,
% $$
% the within class covariance matrix
% $$
% \Sigma_W\Def\ave\limits_{i,k}(h_{i,k}-\mu_k)(h_{i,k}-\mu_k)^T.
% $$
% We standardized variance of noise in the Gaussian model, and the canonical SNR is defined as 
% $$
% \text{SNR}=\ave_{k}||\mu_k-\mu_{k'}||_2,
% $$
% here, $||\cdot||_2$ is the $L_2$ norm.
\vspace{4pt}

\subsection{MP Law and stieltjes Transform}
MP Law is given as follows, 
\begin{theorem}
\label{thm: mpLaw}
(Marchenko Pauster Law) Suppose that the entries $\{w_{ij}\}$ of the matrix $W\in \bbR^{n\times p}$ are $i.i.d.$ complex random variables with mean zero and variance $\sigma^2$, and $n/p\to c\in (0,\infty)$.  Define $S_p=\frac{1}{p}WW^*$, $\lambda_1\geq\lambda_2\geq...\geq\lambda_n$ is the eigenvalue of $S_p$, then the ESD of $S_p$
$$
F^{S_p}\Def\frac{1}{n}\sum_jI(x<\lambda_j)\cvas F_{c,\sigma^2}(x) 
$$
as $p\to\infty$, here $I(\cdot)$ is the indicator function, $F_{c,\sigma^2}$ is the MP Law has the form
$$
F_{c,\sigma^2}(x)=\left\{\begin{aligned}
    &\frac{1}{2\pi xc\sigma^2}\sqrt{(b-x)(x-a)},\ \ \ \ &\text{if}\ a\leq x\leq b,\\
    &0,&\text{otherwise},
\end{aligned}\right.
$$
with an additional point mass of value $1-1/c$ at the origin if $c>1$, where $a=\sigma^2(1-\sqrt{c})^2$ and $b=\sigma^2(1+\sqrt{c})^2$.
\end{theorem}

The powerful mathematical tool to achieve the MP Law is stieltjes Transform, let $\nu$ be a finite measure on the real line with support $\Gamma_\nu$, its stieltjes transform is
$$
s_\nu(z)=\int \frac{1}{x-z}\nu(dx),\ \ z\in\bbC\backslash \Gamma_\nu.
$$
To reduct $\nu$ from Stieltjes transform, we have the equation
$$
\nu(x)=\lim\limits_{v\to0^+}\frac{1}{\pi}\Im s_\nu(x+iv).
$$
Details can be refered in \citep{yao2015sample}.

The Stieltjes transform of standard MP Law satifies equation
$$
s(z)=\frac{1}{1-z-\{c+czs(z)\}},
$$
we can get results in a more generalized settings:
\begin{theorem}
\label{thm: GmpLaw}
(Generalized MP Law) Let $S_p$ be the matrix defined in Theorem \ref{thm: mpLaw}, $(T_p)$ is a sequence of nonnegative Hermitian matrices of size $n\times n$ which is deterministic or independent with $S_p$, and the sequence $(H_p=F^{T_p})$ of the ESD of $(T_p)$ almost surely weakly converges to a nonrandom probability measure $H(t)$, then the ESD $(F^{S_pT_p})$ of $S_pT_p$ weakly converges to a nonrandom probability measure $F_{c,H}$, that its Stieltjes transform is implicitly defined by the equation
$$
s(z)=\int\frac{1}{t(1-c-czs(z))-z}dH(t),\ \ z\in\bbC^+
$$
\end{theorem}

\vspace{4pt}

\subsection{Spike Model}

Suppose that the matrix $T_p$ has the limit ESD $H(t)$, the element $w_{ij}$ in $W$ satifies
$$
Ew_{11}=0,Ew_{11}^2=1,Ew_{11}^4<+\infty
$$
define 
$$
\psi(\alpha)=\psi_{c,H}(\alpha)=\alpha+c\int\frac{t\alpha}{\alpha-t}dH(t),
$$
we say the eigenvalue $\alpha_j$ of $T_p$ with fixed index $j$ is a distant spike eigenvalue if
$$
\psi'(\alpha_j)>0.
$$
Then we have the following theorem,
\begin{theorem}
 The entries $\{w_{ij}\}$ of the matrix $W\in \bbR^{n\times p}$ are $i.i.d.$ complex random variables with mean zero, variance 1 and finite fourth moment, $n/p\to c\in (0,\infty)$.  $S_p=\frac{1}{p}WW^*$, $(T_p)$ is a sequence of nonnegative Hermitian matrices of size $n\times n$ which is deterministic or independent with $S_p$, and the sequence $(H_p=F^{T_p})$ of the ESD of $(T_p)$ almost surely weakly converges to a nonrandom probability measure $H(t)$,  $\lambda_1\geq\lambda_2\geq...\geq\lambda_n$ is the eigenvalue of $S_pT_p$, $\alpha_1\geq\alpha_2\geq...\geq\alpha_n$ is the eigenvalue of $T_p$, suppose that $\alpha_j$ with fixed index $j$ is a distant spike eigenvalue, then as $p\to+\infty$,\newline
 \text{(1)} if $\alpha_1<+\infty$, then $\lambda_j\cvas\psi(\alpha_j)$,\newline
 
\noindent\text{(2)} if $\alpha_j\to+\infty$, then $\lambda_j/\alpha_j\cvas1$.
\end{theorem}

\vspace{4pt}


\subsection{Tracy-Widom Law}

\begin{theorem}
(Tracy-Widom Law) Let $\{w_{i,j}\}$, $i,j=1,2,...,$ be a double array of i.i.d. complex-valued random variables with mean $0$, variance $1$ and finite fourth-order moment. Consider the sample covariance matrix $S_p$ defined same as Theorem \ref{thm: mpLaw}, the eigenvalues of $S_p$: $\lambda_1\geq\lambda_2\geq...\geq\lambda_n$ in a decreasing order. When $n/p\to c$, we have
$$
\lambda_1\cvas (1+\sqrt{c})^2,\quad (order\ 0)
$$
further, define $\mu_{pn}=\frac{1}{p}\{(p-1)^{\frac12}+n^{\frac12}\}^2$ and $\sigma_{pn}=\frac{1}{p}[(p-1)^{\frac12}+n^{\frac12}]\{(p-1)^{-\frac12}+n^{-\frac12}\}^{\frac13}$,
$$
\frac{\lambda_1-\mu_{pn}}{\sigma_{pn}}\cvd F_1,\quad (order\ 1)
$$
where $F_1$ is the Tracy-Widom Law of order 1 whose distribution function is given by 
$$
F_1(s)=\exp{\left\{\int_s^{+\infty}q(x)+(x-s)^2q^2(x)dx\right\}},\quad s\in\bbR,
$$
where $q$ solves the Painleve \uppercase\expandafter{\romannumeral2} differential equation
$$
q''(x)=xq(x)+2q^3(x).
$$
\end{theorem}




==> proof.tex <==
\section{Technique Proof}
In this section, we prove the proposition in section \ref{sec:specCriterion}. 
\subsection{\textbf{Proof of proposition \ref{prop1}}} \label{sec:proof-prop1}

From definition, $\hp_M\left(x\right)=\frac{M}{n\left(b-a\right)}\sum\limits_{i=1}^nI\left(X_i\in B\left(x\right)\right)$, 
$$\begin{aligned}
s_n&=\int_{a}^{b}\left|\hp_M\left(x\right)-p\left(x\right)\right|dx\\
&\leq \int_{a}^{b}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx+\int_{a}^{b}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|dx.
\end{aligned}$$

\vspace{2pt}

We first prove $\int_{a}^{b}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx=O\left(\frac{1}{M}\right)$.

\vspace{2pt}

There exists $x^*\in B_1$ such that $P\left(X_i\in B_1\right)=C\int_{a}^{a+\frac{b-a}{M}}\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{x}dx=C*\frac{b-a}{M}*\frac{\sqrt{\left(b-x^*\right)\left(x^*-a\right)}}{x^*}\leq C*\frac{1}{M}*\sqrt{\frac{1}{M}}$, thus
$$\begin{aligned}
P\left(X_i\in B_1\right)&=O\left(\frac{1}{M^{\frac{3}{2}}}\right),
\end{aligned}$$
similar to get $P\left(X_i\in B_M\right)=O\left(\frac{1}{M^{\frac{3}{2}}}\right)$, then
$$\begin{aligned}
\int_{B_1\cup B_M}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx&\leq \int_{B_1\cup B_M}E\hp_M\left(x\right)+p\left(x\right)dx\\
&=\int_{B_1\cup B_M}\frac{M}{b-a}P\left(X_i\in B_1\cup B_M\right)dx+P\left(X_i\in B_1\cup B_M\right)\\
&=O\left(\frac{1}{M^{\frac{3}{2}}}\right).
\end{aligned}$$


For $\forall x\in B_l$, $l\in\{2,3,...,M-1\}$, there exists $x^*_l\in B_l$ satisfies
$$\begin{aligned}
E\hp_M\left(x\right)&=\frac{M}{b-a}P\left(X_i\in\left(B\left(x\right)\right)\right)\\
&=\frac{\int_{a+\frac{l}{M}\left(b-a\right)}^{a+\frac{l+1}{M}\left(b-a\right)}p\left(u\right)du}{\left(b-a\right)/M}\\
&=p\left(x^*_l\right),
\end{aligned}$$
then for $\forall x\in B_l$, there exists $x^{**}_l$ between $x$ and $x^*_l$, such that 
$$\begin{aligned}
\left|E\hp_M\left(x\right)-p\left(x\right)\right|&=\left|p\left(x^*_l\right)-p\left(x\right)\right|\\
&= \left|p'\left(x^{**}_l\right)\left(x^{*}_l-x\right)\right|\\
&\leq C*\frac{\left|x^{**}_l-\left(x^{**}_l-a\right)\left(b-x^{**}_l\right)\right|}{\sqrt{\left(x^{**}_l-a\right)\left(b-x^{**}_l\right)}\left(x^{**}_l\right)^2}*\left|x^*_l-x\right|\\
&\leq\frac{C}{\sqrt{lM}},
\end{aligned}$$
$C$ is an absolute value. Then 
$$\begin{aligned}
\int_{B_1^C\cap B_M^C}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx&=\sum\limits_{l=2}^{M-1}\int_{B_l}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx\\
&\leq \sum\limits_{l=2}^{M-1}\int_{B_l}\frac{1}{\sqrt{l}}\cdot \frac{C}{\sqrt M}dx\\
&=\sum\limits_{l=2}^{M-1}\frac{1}{\sqrt{l}}\cdot \frac{C}{\sqrt M}\cdot\frac{1}{M}\\
&=O\left(\frac{1}{M}\right).
\end{aligned}$$
Thus
$$\begin{aligned}
\int_{a}^{b}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx&=\int_{B_1\cup B_M}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx\\
&+\int_{B_1^C\cap B_M^C}\left|E\hp_M\left(x\right)-p\left(x\right)\right|dx\\
&=O\left(\frac1M\right).
\end{aligned}$$

We next prove that $\int_{a}^{b}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|dx=O_P\left(\sqrt{\frac{M\log n}{n}}\right)$.




$$\begin{aligned}
P\left(\sup\limits_x\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|>\varepsilon\right)&=P\left(M\cdot\max\limits_{l=1,...,M}\frac{1}{n}\left|\sum\limits_{i=1}^nI\left(X_i\in B_l\right)-nP\left(X_i\in B_l\right)\right|>\varepsilon\right)\\
&=P\left(\max\limits_{l=1,...,M}\frac{1}{n}\left|\sum\limits_{i=1}^nI\left(X_i\in B_l\right)-nP\left(X_i\in B_l\right)\right|>\frac{\varepsilon}{M}\right)\\
&\leq \sum\limits_{l=1}^{M}P\left(\frac{1}{n}\left|\sum\limits_{i=1}^nI\left(X_i\in B_l\right)-nP\left(X_i\in B_l\right)\right|>\frac{\varepsilon}{M}\right)
\end{aligned}$$
Note that $P\left(X_i\in B_l\right)=O\left(1/M\right)$, by Berstein inequality, 
$$\begin{aligned}
\sum\limits_{l=1}^{M}P\left(\frac{1}{n}\left|\sum\limits_{i=1}^nI\left(X_i\in B_l\right)-nP\left(X_i\in B_l\right)\right|>\frac{\varepsilon}{M}\right)
&\leq \sum\limits_{l=1}^{M}e^{-C\frac{\frac{n^2\varepsilon^2}{M^2}}{\frac{n}{M}+\frac{n\varepsilon}{3M}}}\\
&\leq Me^{-C\frac{n\varepsilon}{M}}
\end{aligned}$$
for some constant $C>0$, set $\varepsilon=\sqrt{\frac{M\log n}{n}}$, we achieve 
$$
\sup\limits_{x\in\left[a,b\right]}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|=O_P\left(\sqrt{\frac{M\log n}{n}}\right),
$$
which implies given $\forall$ $\varepsilon_0>0$, there $\exists R>0$, such that
$$
P\left(\sqrt{\frac{n}{M\log n}}\sup\limits_{x\in\left[a,b\right]}|\hp_M\left(x\right)-E\hp_M\left(x\right)|>R\right)<\varepsilon_0,
$$
for $\int_{a}^{b}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|dx$, there exists $x_n$ satisfies
$$
\left|\hp_M\left(x_n\right)-E\hp_M\left(x_n\right)\right|\left(b-a\right)\geq \int_{a}^{b}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|dx,
$$
then
$$\begin{aligned}
\varepsilon_0&>P\left(\sqrt{\frac{n}{M\log n}}\sup\limits_{x\in\left[a,b\right]}|\hp_M\left(x\right)-E\hp_M\left(x\right)|>R\right)\\
&\geq P\left(\sqrt{\frac{n}{M\log n}}|\hp_M\left(x_n\right)-E\hp_M\left(x_n\right)|\left(b-a\right)>R\left(b-a\right)\right)\\
&\geq P\left(\sqrt{\frac{n}{M\log n}}\int_{a}^{b}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|dx>R\left(b-a\right)\right)\\
\end{aligned}$$
Thus we achieve
$$
\int_{a}^{b}\left|\hp_M\left(x\right)-E\hp_M\left(x\right)\right|dx=O_P\left(\sqrt{\frac{M\log n}{n}}\right),
$$
which proves the proposition.
\newpage








\subsection{\textbf{Proof of proposition \ref{prop2}}} \label{sec:proof-prop2}

Recall $X_{\left(i\right)}$ is the order statistics. For $\forall \varepsilon>0$, $\exists R>0$ such that 
$$\begin{aligned}
P\left(n^{\frac{2}{3}}\left(X_{\left(1\right)}-a\right)>R\right)&=\prod\limits_{i=1}^nP\left(X_{i}-a>R/n^{\frac23}\right)\\
&=\left(1-\int_a^{a+\frac{R}{n^{\frac23}}}p\left(x\right)dx\right)^n\\
&\sim\left(1-C\int_a^{a+\frac{R}{n^{\frac23}}}\sqrt{x-a}dx\right)^n\\
&=\left(1-CR^{\frac32}/n\right)^n\\
&<\varepsilon
\end{aligned}$$
as $n\to\infty$, then $X_{\left(1\right)}-a=O_P\left(n^{-\frac{2}{3}}\right)$, similar to get $b-X_{\left(n\right)}=O_P\left(n^{-\frac23}\right)$, which implies same rate as Tracy Widom Law.

$$
\hs_n\leq s_n+\int_a^b|\hp\left(x\right)-p\left(x\right)|dx,
$$
The only thing is to prove
$$
\int_a^b|\hp\left(x\right)-p\left(x\right)|dx=O_P\left(n^{-\frac13}\right).
$$

Indeed, set $C_0=2\pi\sigma^2c$, $\hC_0=\frac{\pi\left(\sqrt{X_{\left(n\right)}}-\sqrt{X_{\left(1\right)}}\right)^2}{2}$, we have
$$\begin{aligned}
\int_a^b\left|\hp\left(x\right)-p\left(x\right)\right|dx&=\int_a^b\left|\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{C_0x}-\frac{\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}}{\hC_0x}I\left(\left[X_{\left(1\right)},X_{\left(n\right)}\right]\right)\right|dx\\
&\leq \int_a^b\left|\frac{1}{\hC_0}\right|\cdot\left|\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{x}-\frac{\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}}{x}I\left(\left[X_{\left(1\right)},X_{\left(n\right)}\right]\right)\right|dx\\
&+\left|\frac{1}{C_0}-\frac{1}{\hC_0}\right|\Def P_1+P_2,
\end{aligned}$$
where $P_1=\int_a^b\left|\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{C_0x}-\frac{\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}}{\hC_0x}I\left(\left[X_{\left(1\right)},X_{\left(n\right)}\right]\right)\right|dx$, $P_2=\left|\frac{1}{C_0}-\frac{1}{\hC_0}\right|$. Note that $\hC_0\cvp C_0>0$, by continuous mapping, $\frac{1}{\hC_0}\cvp \frac{1}{C_0}>0$, thus $\frac{1}{\hC_0}=O_P\left(1\right)$. Then for $P_2=\left|\frac{1}{C_0}-\frac{1}{\hC_0}\right|$, we have 
$$\begin{aligned}
\left|\frac{1}{C_0}-\frac{1}{\hC_0}\right|&=\frac{\pi\left(\left(\sqrt{b}-\sqrt{a}\right)^2-\left(\sqrt{X_{\left(n\right)}}-\sqrt{X_{\left(1\right)}}\right)^2\right)}{2C_0\hC_0}\\
&\leq O_P\left(1\right)\cdot O_P\left(\sqrt{b}-\sqrt{X_{\left(n\right)}}+\sqrt{X_{\left(1\right)}}-\sqrt{a}\right)\\
&=O_P\left(n^{-\frac{2}{3}}\right),
\end{aligned}$$
for the first part, the integration can be separated as 
$$\begin{aligned}
P_1&=\int_a^{X_{\left(1\right)}}\left|\frac{1}{\hC_0}\right|\cdot\left|\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{x}-\frac{\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}}{x}I\left(\left[X_{\left(1\right)},X_{\left(n\right)}\right]\right)\right|dx\\
&+\int_{X_{\left(1\right)}}^{X_{\left(n\right)}}\left|\frac{1}{\hC_0}\right|\cdot\left|\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{x}-\frac{\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}}{x}I\left(\left[X_{\left(1\right)},X_{\left(n\right)}\right]\right)\right|dx\\
&+\int_{X_{\left(n\right)}}^b\left|\frac{1}{\hC_0}\right|\cdot\left|\frac{\sqrt{\left(b-x\right)\left(x-a\right)}}{x}-\frac{\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}}{x}I\left(\left[X_{\left(1\right)},X_{\left(n\right)}\right]\right)\right|dx\\
&\Def P_{11}+P_{12}+P_{13},
\end{aligned}$$
there exists $x^*\in \left(a,X\left(1\right)\right)$ such that 
$$\begin{aligned}
P_{11}=\left|\frac{1}{\hC_0}\right|\cdot\left|\frac{\sqrt{\left(b-x^*\right)\left(x^*-a\right)}}{x^*}\right|\left(X_{\left(1\right)}-a\right)=O_P\left(n^{-\frac23}\right),
\end{aligned}$$
similar to get 

$$\begin{aligned}
P_{13}=O_P\left(n^{-\frac23}\right),
\end{aligned}$$

$$\begin{aligned}
P_{12}&=O_P\left(\int_{X_{\left(1\right)}}^{X_{\left(n\right)}}\left|\frac{\left(b-a-X_{\left(n\right)}+X_{\left(1\right)}\right)x-ab+X_{\left(n\right)}X_{\left(1\right)}}{x\left(\sqrt{\left(b-x\right)\left(x-a\right)}+\sqrt{\left(X_{\left(n\right)}-x\right)\left(x-X_{\left(1\right)}\right)}\right)}\right|dx\right)\\
&=O_P\left(\int_{X_{\left(1\right)}}^{X_{\left(n\right)}}\left|\frac{b-a-X_{\left(n\right)}+X_{\left(1\right)}}{\sqrt{\left(b-x\right)\left(x-a\right)}}\right|dx\right)+O_P\left(\int_{X_{\left(1\right)}}^{X_{\left(n\right)}}\left|\frac{ab-X_{\left(n\right)}X_{\left(1\right)}}{x\sqrt{\left(b-x\right)\left(x-a\right)}}\right|dx\right),
\end{aligned}$$
by simple integration calculation, we have 
$$
P_{12}=O_P\left(n^{-\frac13}\right).
$$

Thus, 
$$
\int_a^b|\hp\left(x\right)-p\left(x\right)|dx=O_P\left(n^{-\frac13}\right),
$$
which proves the proposition.


==> table1.tex <==


\begin{figure}[htbp]

\centering
\includegraphics[width=2.2in]{picture/SNR_Acc.png}
%\caption{fig1}

\caption{:~~1  }
\end{figure}

\begin{table}[htbp]
\renewcommand\tabcolsep{10pt}
\begin{tabular}{ccccc}
              & \multicolumn{2}{c}{$\delta=0.24$} & \multicolumn{2}{c}{$\delta=0.24$} \\
              & FC2             & FC3             & FC2             & FC3             \\
NN1+$\calD_1$ & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}               \\
              & FC1             & FC2             & FC1             & FC2             \\
NN2+$\calD_1$ & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                \\
              & \multicolumn{2}{c}{$\delta=0.24$} & \multicolumn{2}{c}{$\delta=0.24$} \\
              & FC1             & FC2             & FC1             & FC2             \\
NN1+$\calD_2$ & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                \\
              & FC1             & FC2             & FC1             & FC2             \\
NN2+$\calD_2$ & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                &\begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}                & \begin{minipage}[b]{0.2\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=1.4\linewidth]{picture/Gaps/NN1+D1.png}}
	\end{minipage}               
\end{tabular}
\end{table}













\begin{table}[h]
\centering
\linespread{0.5} 
\renewcommand\tabcolsep{-25pt}
\begin{tabular}{ccccc}
  & \multicolumn{2}{c}{$\delta=0.5$} & \multicolumn{2}{c}{$\delta=0.7$} \\
D1 & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}              & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}             \\
D2 & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}              & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}             &\subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}              \\
  & \multicolumn{2}{c}{$\delta=0.5$} & \multicolumn{2}{c}{$\delta=0.5$} \\
D3 & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}              &\subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}              \\
D4 & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}              & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}               & \subfigure[$\lambda_{\max}$]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.5in]{picture/watchepochs/Max.png}
%\caption{fig2}
\end{minipage}%
}             
\end{tabular}
\end{table}




==> table2.tex <==
\vspace{-30pt}
\section{Numeric Experiments} \label{sec: simulation}




\begin{table}[htbp]
\centering
\caption{~~\textbf{NN2+}$\calD_1$: The results of ESD types in different layers with different SNR, and the number of spikes is related to Classes number. }
\label{tb:NN2D1}
\begin{tabular}{|c|c|c|c|}
\hline
Classes Number       & Layer                & Transition Period & TP Range+ESD Type                                                                                                         \\ \hline
\multirow{6}{*}{K=2} & \multirow{3}{*}{FC1} & Heavy Tail        & {[}0.005-0.015{]}: HT(0,1)                                                                                                                         \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.02-0.055{]}: HT(1,1)$\to$MPB(1,1)                                                                               \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.06,0.235{]}: LT(1,1)\\ {[}0.24,0.4{]}: LT(0,1)\end{tabular}                              \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                                                         \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                         \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.005,0.4{]}: LT(1,1)                                                                                                \\ \hline
\multirow{6}{*}{K=5} & \multirow{3}{*}{FC1} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.005,0.015{]}: HT(0,1)\\ {[}0.02,0.035{]}: HT(4,1)\\ {[}0.04,0.045{]}: HT(0,5)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.05,0.12{]}: HT(1,4)$\to$MPB(1,4)                                                                                 \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.125,0.4{]}: LT(1,4)                                                                                                \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                                                         \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.005,0.025{]}: HT(1,4)$\to$MPB(1,4)                                                                               \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.03,0.38{]}: LT(1,4)\\ {[}0.385,0.4{]}: LT(0,5)\end{tabular}                               \\ \hline
\multirow{6}{*}{K=8} & \multirow{3}{*}{FC1} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.005,0.025{]}: HT(0,1)\\ {[}0.03,0.06{]}: HT(7,1)\\ {[}0.065{]}: HT(0,8)\end{tabular}       \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.07,0.135{]}: HT(1,7)$\to$MPB(1,7)                                                                                \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.135,0.4{]}: LT(1,7)                                                                                                 \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                                                         \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.005,0.095{]}: MPB(1,7)                                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.1,0.24{]}: LT(1,7)\\ {[}0.245,0.4{]}: LT(0,8)\end{tabular}                                \\ \hline
\end{tabular}

\end{table}

\newpage



\begin{table}[htbp]
\centering
\caption{~~\textbf{NN2+}$\calD_2$: The results of ESD types in different layers with different SNR, and the number of spikes is related to Classes number.}
\label{tb:NN2D2}
\begin{tabular}{|c|c|c|c|}
\hline
Classes Number       & Layer                & Transition Period & TP Range+ESD Type                                                                                            \\ \hline
\multirow{6}{*}{K=2} & \multirow{3}{*}{FC1} & Heavy Tail        & {[}0.08,0.16{]}: HT(0,1)                                                                                      \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.24-1.52{]}: HT(1,1)$\to$MPB(1,1)                                                                    \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}1.6,1.92{]}: LT(1,1)\\ {[}2,4.8{]}: LT(0,1)\end{tabular}                     \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,0.48{]}: MPB(1,1)                                                                                  \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.56,4.8{]}: LT(0,1)                                                                                      \\ \hline
\multirow{6}{*}{K=5} & \multirow{3}{*}{FC1} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,0.48{]}: HT(0,0)\\ {[}0.56{]}: HT(0,1)\\ {[}0.64,0.88{]}: HT(0,5)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.96,2.24{]}: HT(1,4)$\to$MPB(1,4)                                                                    \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}2.32,2.48{]}: LT(1,4)\\ {[}2.56,4.8{]}: LT(0,4)\end{tabular}                 \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,2.16{]}: HT(0,4) $\to$ MPB(1,4)                                                                                    \\ \cline{3-4} 
                     &                      & Light Tail        & {[}2.24,4.8{]}: LT(1,4)                                                                                   \\ \hline
\multirow{6}{*}{K=8} & \multirow{3}{*}{FC1} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,0.96{]}: HT(0,0)\\ {[}1.04,1.12{]}: HT(0,8)\end{tabular}                      \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}1.2,2.72{]}: HT(1,7)$\to$MPB(1,7)                                                                     \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}2.8,3.04{]}: LT(1,7)\\ {[}3.12,4.8{]}: LT(0,7)\end{tabular}                  \\ \cline{2-4} 
                     & \multirow{3}{*}{FC2} & Heavy Tail        & -                                                                                                            \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,2.4{]}:HT(0,7)$\to$ MPB(1,7)                                                                                   \\ \cline{3-4} 
                     &                      & Light Tail        & {[}2.48,4.8{]}: LT(1,7)$\to$LT(0,8)                                                                         \\ \hline
\end{tabular}

\end{table}


\begin{table}[htbp]
\centering
\caption{~~\textbf{NN1+}$\calD_1$: The results of ESD types in different layers with different SNR. }
\label{tb:NN1D1}
\begin{tabular}{|c|c|c|c|}
\hline
Classes Number       & Layer                & Transition Period & TP Range+ESD Type                                                                                                    \\ \hline
\multirow{9}{*}{K=2} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.03{]}: HT(0,1)\\ {[}0.04-0.09{]}: HT(0,2)\end{tabular}                             \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.1-0.44{]}: HT(1,1)$\to$MPB(1,1)                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.45-2{]}: LT(1,1)                                                                                              \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & -                                                                                                                    \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.01,0.29{]}: MPB(1,1)                                                                                          \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.3,0.38{]}: LT(1,1)\\ {[}0.39,2{]}: LT(0,1)\end{tabular}                            \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                    \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                    \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.01,2{]}: LT(0,1)                                                                                                \\ \hline
\multirow{9}{*}{K=5} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.15{]}: HT(0,1)\\ {[}0.16,0.2{]}: HT(4,1)\\ {[}0.2,0.28{]}: HT(0,5)\end{tabular}  \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.28,0.66{]}: HT(1,4)$\to$MPB(1,4)                                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.67,1.04{]}: LT(1,4)\\ {[}1.04,2{]}: LT(0,5)\end{tabular}                          \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & -                                                                                                                    \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.01,0.59{]}: HT(1,4)$\to$MPB(1,4)                                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.6,1.9{]}: LT(1,4)\\ {[}1.95,2{]}: LT(0,5)\end{tabular}                               \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                    \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                    \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.01,2{]}: LT(0,4)                                                                                                  \\ \hline
\multirow{9}{*}{K=8} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.01,0.19{]}: HT(0,1)\\ {[}0.2,0.25{]}: HT(7,1)\\ {[}0.26,0.36{]}: HT(0,8)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.37-0.72{]}: HT(1,7)$\to$MPB(1,7)                                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.73,1.01{]}: LT(1,7)\\ {[}1.02,1.9{]}: LT(0,8)\\ {[}1.95,2{]}: LT(0,7)\end{tabular}      \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & {[}0.01,0.32{]}: HT(0,8)                                                                                               \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.32,0.62{]}: HT(1,7)$\to$MPB(1,7)                                                                            \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.63,1.15{]}: LT(1,7)\\ {[}1.16,1.95{]}: LT(0,8)\\ {[}2{]}: LT(0,7)\end{tabular}         \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                    \\ \cline{4-4} 
                     &                      & Bulk Transition   & -                                                                                                                    \\ \cline{4-4} 
                     &                      & Light Tail        & {[}0.01,2{]}: LT(0,7)                                                                                                 \\ \hline
\end{tabular}

\end{table}










\begin{table}[htbp]
\centering
\caption{~~\textbf{NN1+}$\calD_2$: The results of ESD types in different layers with different SNR. }
\label{tb:NN1D2}
\begin{tabular}{|c|c|c|c|}
\hline
Classes Number       & Layer                & Transition Period & TP Range+ESD Type                                                                                                     \\ \hline
\multirow{9}{*}{K=2} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,0.024{]}: HT(0,1)\\ {[}0.32,0.4{]}: HT(0,2)\end{tabular}                              \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.48-2.16{]}: HT(1,1)$\to$MPB(1,1)                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & {[}2.24,4.8{]}: LT(1,1)                                                                                            \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & -                                                                                                                     \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,1.44{]}: HT(1,1)$\to$MPB(1,1)                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}1.52,2.64{]}: LT(1,1)\\ {[}2.72,4.8{]}: LT(0,1)\end{tabular}                          \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                     \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                     \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.08,4.8{]}: LT(0,1)                                                                                               \\ \hline
\multirow{9}{*}{K=5} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,0.48{]}: HT(0,1)\\ {[}0.56,0.64{]}: HT(4,1)\\ {[}0.72,1.04{]}: HT(0,5)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}1.12,3.2{]}: HT(1,4)$\to$MPB(1,4)                                                                              \\ \cline{3-4} 
                     &                      & Light Tail        & {[}3.28,4.8{]}: LT(1,4)                                                                                            \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & -                                                                                                                     \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}0.08,2.72{]}: HT(1,4)$\to$MPB(1,4)                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & {[}2.8,4.8{]}: LT(1,4)                                                                                             \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                     \\ \cline{3-4} 
                     &                      & Bulk Transition   & -                                                                                                                     \\ \cline{3-4} 
                     &                      & Light Tail        & {[}0.08,4.8{]}: LT(0,4)                                                                                               \\ \hline
\multirow{9}{*}{K=8} & \multirow{3}{*}{FC2} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,0.56{]}: HT(0,1)\\ {[}0.64,0.96{]}: HT(7,1)\\ {[}1.04,1.36{]}: HT(0,8)\end{tabular} \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}1.44,3.52{]}: HT(1,7)$\to$MPB(1,7)                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & \begin{tabular}[c]{@{}c@{}}{[}3.6,4.64{]}: LT(1,7)\\ {[}4.8{]}: LT(0,8)\end{tabular}                                 \\ \cline{2-4} 
                     & \multirow{3}{*}{FC3} & Heavy Tail        & \begin{tabular}[c]{@{}c@{}}{[}0.08,1.12{]}: HT(7,1)\\ {[}1.12,1.44{]}: HT(0,8)\end{tabular}                           \\ \cline{3-4} 
                     &                      & Bulk Transition   & {[}1.52,3.12{]}: HT(1,7)$\to$MPB(1,7)                                                                             \\ \cline{3-4} 
                     &                      & Light Tail        & {[}3.12,4.8{]}: LT(1,7)                                                                                            \\ \cline{2-4} 
                     & \multirow{3}{*}{FC4} & Heavy Tail        & -                                                                                                                     \\ \cline{4-4} 
                     &                      & Bulk Transition   & -                                                                                                                     \\ \cline{4-4} 
                     &                      & Light Tail        & {[}0.08,4.8{]}: LT(0,7)                                                                                                \\ \hline
\end{tabular}

\end{table}

